Modelling the prompt optical emission of GRB 180325A: the evolution of a spike from the optical to gamma-rays

The transition from prompt to the afterglow emission is one of the most exciting and least understood phases in gamma-ray bursts (GRBs). Correlations among optical, X-ray and gamma-ray emission in GRBs have been explored, to attempt to answer whether the earliest optical emission comes from internal and/or external shocks. We present optical photometric observations of GRB 180325A collected with the TAROT and RATIR ground-based telescopes. These observations show two strong optical flashes with separate peaks at $\sim50\;$s and $\sim120\;$s, followed by a temporally extended optical emission. We also present X-rays and gamma-ray observations of GRB 180325A, detected by the Burst Alert Telescope (BAT) and X-ray Telescope (XRT), on the Neil Gehrels Swift observatory, which both observed a narrow flash at $\sim80\;$s. We show that the prompt gamma- and X-ray early emission shares similar temporal and spectral features consistent with internal dissipation within the relativistic outflow (e.g. by internal shocks or magnetic reconnection), while the early optical flashes are likely generated by the reverse shock that decelerates the ejecta as it sweeps up the external medium.

==> apendixstep.tex <==
% \appendix sets everything in single column. So, let's fake it. This at least fixes the section labels.
\renewcommand{\thesection}{\Alph{section}}
\setcounter{section}{0}

\section{Step function velocity variation} 
\label{app:step}

We consider a free-streaming flow injected at $x=0$ with velocity $\beta$ and mass-loss rate $\dot m$. We assume a velocity variation (see Figure \ref{fig:step}) with a slow flow injected in the interval $[-\Delta \tau_s, 0]$ and
 a fast flow injected in the interval $[0, \Delta \tau_f]$.
 The material injected at time $\tau$ arrives to the position $x$ at the lab-frame time $t$ according to the free-streaming 
 relation
\begin{equation}
    \beta(x,t) = \beta(0,\tau) = \frac{x}{c\left(t-\tau\right)},
\label{eq:free_st}
\end{equation}
where $c$ is the speed of light.
Since the injection velocity varies with time,  a two-shock WS is formed. This WS
is fed by a fast upstream and a slow downstream material. 
A WS is formed at the position $x_{\rm ws}$ at a time $\tau_i$ given by the condition \citep{2000MNRAS.313..656C}
\begin{equation}
\frac{x_{\rm ws}}{c} = \left[\frac{\beta^2}{d \beta/d \tau} \right]_{\min}.
\label{eq:WS0}
\end{equation}
For the assumed step function variability $x_{\rm ws} = 0$ at time $t=0$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\centering
\includegraphics[angle=0,width=0.45\textwidth]{Figure7.pdf} 
\caption{Injection velocity $\beta(\tau)$ as a function of time $\tau$ at the position of the shell collision. The time intervals 
$\Delta \tau_s$ and $\Delta \tau_f$ represent the duration of the injection of the fast and slow material.}
\label{fig:step}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 According to \cite{2013MNRAS.430.2703C}, the WS  has a constant velocity phase with an intermediate speed corresponding to a Lorentz factor
\begin{equation}
\gamma_{ws0}=
\frac{\lambda+1}{ 
\sqrt{ \left( {\lambda/ \gamma_f} \right)^2  + 2 \lambda\left(1-\beta_s\beta_f\right) +
1/\gamma_s^2  } } .
\label{eq:gamma0}
\end{equation}
In this equation one defines
\begin{equation}
\lambda = \sqrt{\frac{b r}{a}},
\label{eq:lambda}
\end{equation}
where the velocity ratio, the mass-loss ratio, and the gamma ratio are given by
\begin{equation}
 a=\beta_f/\beta_s, \quad b=\dot m_f/\dot m_s, 
\quad r= \gamma_f/\gamma_s.
\end{equation}



\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figure8.pdf}
\caption{Qualitative temporal evolution of the working surface Lorentz factor for Case I (green line) and Case II (red line). The initial constant velocity for the two cases is shown in blue. 
}
\label{fig5}
\end{figure}



The duration of the constant velocity phase and the subsequent evolution of the WS depends on which material runs out first.
In case I, the constant velocity phase ends when the fast material is completely incorporated into  the WS, at a time $ t_{\rm c}^{I}$  given by 
\begin{equation}
 t_{\rm c}^{I} = \frac{a \left( \lambda + 1 \right)}{a-1} \Delta \tau_f
 \approx
  \frac{2\gamma_s^2 }{1-\gamma_s^2/\gamma_f^2}  \left( \lambda + 1 \right) \Delta \tau_f .
\label{tcI}
\end{equation}
Afterwards, the WS decelerates such that the 
Lorentz factor  $\gamma_{\rm ws}^I(t)$ varies with time as
\newcommand{\T}{\mathcal{T}}
\begin{equation}
\gamma_{\rm ws}^I= \gamma_s \left( \frac{\T^2 + 4 \beta_s \T + 4}{\T^2 - 4 } \right),
\label{eq:gammaI}
\end{equation}
where $\T(t)$ is a function of time given by the transcendental equation 
\begin{equation}
 \frac{\T^2}{2} + 4 \beta_s \T + 4 \ln{\T} = \frac{4 C^{I} }{ \beta_s \gamma_s^3} \frac{t}{\Delta \tau_f} + D^{I},
 \label{eq:calTI}
\end{equation}
 where the constants $C^I$ and $D^I$ are given by equations (21) and (24) of \cite{2013MNRAS.430.2703C}.
 The deceleration phase ends at a time $t_s$, when the WS completely engulfs the slow moving material. From the 
 free-streaming relation eq. (\ref{eq:free_st}), $t_s$ is given by the condition
\begin{equation}
 v_s \;(t_s + \Delta \tau_s) =
  R_{\rm ws}(t_s)
 % v_{ws,0} \;t_c^{I} + \int_{t_c^{I}}^{t_{s}} v_{ws}^{I}(t) \;dt .
\end{equation}

 
 In case II, the constant velocity phase ends
 when the slow material is completely incorporated into  the WS, at a time $ t_{\rm c}^{II}$
 given by 
  \begin{equation}
 t_{\rm c}^{II} = \frac{  \lambda + 1}{\lambda (a-1)}\Delta \tau_s
 \approx
  \frac{2\gamma_s^2}{1-\gamma_s^2/\gamma_f^2}  \frac{\lambda + 1}{\lambda}  \Delta \tau_s
\label{tcII}
\end{equation}
 The WS then accelerates  such that
the Lorentz factor $\gamma_{\rm ws}^{II}(t)$ is
\begin{equation}
\gamma_{\rm ws}^{II}= \gamma_f \left( \frac{\T^2 - 4 \beta_f \T + 4}{\T^2 - 4 } \right),
\label{eq:gammaII}
\end{equation}
where $\T(t)$ is given by the transcendental equation 
\begin{equation}
 \frac{\T^2}{2} - 4 \beta_f \T + 4 \ln{\T} = \frac{4 C^{II} }{\beta_f \gamma_f^3} \frac{t}{\Delta \tau_s} + D^{II},
 \label{eq:calTII}
 \end{equation}
 where the constants $C^{II}$ and $D^{II}$ are given by equations (33) and (36) of \cite{2013MNRAS.430.2703C}.

The acceleration phase ends at a time $t_f$, when the WS completely engulfs the fast moving material, i.e. when 
\begin{equation}
 v_{f} \;(t_{f} - \Delta \tau_{f}) = R_{\rm ws} (t_s)
 %v_{ws,0} \;t_c^{II} + \int_{t_c^{II}}^{t_{f}} v_{ws}^{II}(t) \;dt\;.
 \label{eq:tfast}
\end{equation}

In summary, the collision of the two shells forms a WS that has
an initial constant velocity phase with a Lorentz factor $\gamma_{ws0}$ 
given by equation (\ref{eq:gamma0}). In case I, 
after a critical time $t_c^I$, the WS decelerates with a Lorentz factor $\gamma_{\rm ws}^I(t)$ 
given by equation (\ref{eq:gammaI}); in case II, after a critical time $t_c^{II}$, the  WS accelerates 
with a  Lorentz factor $\gamma_{\rm ws}^{II}(t)$  given by equation (\ref{eq:gammaII}). 
Finally, the velocity of the WS becomes constant when all the material has been incorporated. (see Figure \ref{fig5} for a schematic representation of the evolution of the Lorentz factor of the WS). 
 
 This model can also be applied to the case of a fast shell that runs into a static medium. In this case,
 consider a static medium with a density $\rho_s$ and $\beta_s =0$, and a fast shell with density $\rho_f$
 and a velocity $\beta_f$. Since the mass-loss-rate is $\dot m \propto \rho \beta$ , the parameter $\lambda$
 can be written as $  \lambda = (\rho_f \gamma_f/\rho_s)^{1/2}$. Then, the phase of constant velocity has
 \begin{equation}
 \gamma_{ws0} = \frac{\lambda+1}{ 
\sqrt{ \left( {\lambda/ \gamma_f} \right)^2  + 2 \lambda +
1 } } .
 \end{equation}
 This phase ends at the time $t_c^I$ when all the fast material has been incorporated to the WS. From then on,
 the WS decelerates continuously with a Lorentz factor given by eq. (\ref{eq:gammaI}) and approaches asymptotically 
 to rest (see case I in Fig. 3 of \cite{2013MNRAS.430.2703C}).
 
%=======================================
%\section{Calculation of the spectrum}
%\label{apB}
%=========================================

%Given the dynamical evolution of the forward and reverse shocks (Section \ref{sec:shock}), we compute in this Section the resulting emission. We assume it is produced by synchrotron radiation. 

%From the Taub relativistic shock-jump conditions we compute the post-shock energy density $e_{\rm ps}$, density $\rho_{\rm ps}$ and velocity $v_{\rm ps}$ as a function of the the pre-shock density and the velocities of the fast and slow material ejected from the central engine. Thus, the post-shock physical variables will evolve with time as the working surface acelerates or decelerates as discussed in Section \ref{sec:shock}.

%To compute the synchrotron radiation, we assume that a fraction $\chi_e$ of the post-shock electrons are accelerated to relativistic speeds, forming a population of electrons $N(\gamma_e) \propto \gamma_e^{-p}$, where $p$ is the power-index of the population of non-thermal electrons accelerated by the shock, and the distribution starts at $\gamma_e>\gamma_m$, being
%
%\begin{equation}
%  \gamma_m(t) = \frac{p-2}{p-1} 
%      \frac{\epsilon_e e_{\rm %ps}(t)}{\chi_e n_{\rm ps}(t) m_e c^2}
%\end{equation}
%
%the minimum Lorentz factor of the accelerated electrons. 
%The energy of the accelerated electrons and the post-shock magnetic field are taken as a fraction $\epsilon_e$ and $\epsilon_B $ of the post-shock thermal energy.

%As the electrons cool, the electron population changes with time as
%
%\begin{equation}
%  N(\gamma_e,t) = N(\gamma_e) \left(1- \frac{\gamma_m(t)}{\gamma_{\rm max}(t)} \right)^{p-2}\;,
%\end{equation}
%
%where $\gamma_{\rm max} = 3 m_e c/(4 \sigma_T e_{\rm th} \epsilon_B t)$.
%As electrons are advected with the flow in the post-shock region, the synchrotron emissivity is thus computed (during a time larger than the cooling time) as 
%
%\begin{equation}
% P(\nu)=\int N(\gamma_e,t) P_{\rm sync}(\gamma_e,\nu) d\gamma_e\;,
%\end{equation}
%
%where $P_{\rm sync}(\gamma_e,\nu)$ is the synchrotron specific power of an electron with Lorentz factor $\gamma_e$ (e.g., \citealt{decolle12}).

%We compute the flux at different polar angles $\theta$ (measured with respect to the direction of motion of the jet) and add each contribution to the corresponding time range in the observing frame, by using the relation $t_{\rm obs}= t - r \cos \theta/c$, being $r$ the radial distance from the central engine.

%In synthesis, light curve and spectrum are computed as a function of the following parameters: the Lorentz factors $\gamma_f(t)$ and $\gamma_s(t)$ of the fast and slow unshocked material, the mass-loss rates (or the density) $\dot{m}_f$,  $\dot{m}_s$, and the duration of injection of the fast and slow material $\Delta \tau_f$ and $\Delta \tau_s$.  In addition, the synchrotron radiation calculation is parameterized as a function of the microphysical parameters $\epsilon_e$, $\epsilon_B$ and $p$.
%In the following, we fix the values of $\epsilon_e=\epsilon_B=0.1$ and $p=3$ and change the other parameters to explore different physical scenarios as described below.

